Towards More Realistic Extraction Attacks: An Adversarial Perspective

Language models are prone to memorizing their training data, making them vulnerable to extraction attacks. While existing research often examines isolated setups, such as a single model or a fixed prompt, real-world adversaries have a considerably larger attack surface due to access to models across various sizes and checkpoints, and repeated prompting. In this paper, we revisit extraction attacks from an adversarial perspective -- with multi-faceted access to the underlying data. We find significant churn in extraction trends, i.e., even unintuitive changes to the prompt, or targeting smaller models and earlier checkpoints, can extract distinct information. By combining multiple attacks, our adversary doubles ($2 \times$) the extraction risks, persisting even under mitigation strategies like data deduplication. We conclude with four case studies, including detecting pre-training data, copyright violations, extracting personally identifiable information, and attacking closed-source models, showing how our more realistic adversary can outperform existing adversaries in the literature.

==> tables/table_similarity_metrics.tex <==
\begin{table*}
    \centering
    % \small
    \begin{tabular}{p{0.36\linewidth}p{0.27\linewidth}p{0.27\linewidth}}
         \toprule
         \textbf{Metric} & \textbf{Advantages} & \textbf{Disadvantages} \\
         % \midrule
         % \cmidrule(lr){1-4}\cmidrule(lr){5-10}\cmidrule(lr){11-12}
         \midrule
         \textbf{Verbatim match:} Exact overlap between generated and original text. & Strong evidence of memorization. No hyperparameter. & Highly brittle to noisy generation. Limited in scope. \\
         \addlinespace[0.5em]
         \textbf{Levenshtein Ratio:} Minimum single-character edits (insertions, deletions or substitutions) between two sequences. & Can recognize fragments of extracted information. Robust to noise. Continuous metric. & Ambiguity at smaller thresholds due to coincidental similarity. Lacks interpretability. \\
         \addlinespace[0.5em]
         \textbf{Longest Common Substring (LCS):} Longest common substring present in both sequences. & Compromise between edit distance metrics and verbatim match. Interpretable. & Does not account for the presence of multiple substrings. \\
         \addlinespace[0.5em]
         \textbf{$n$-gram similarity:} Ratio of $n$-grams common between two sequences. & Granular. Can also detect multiple fragments of information. & Highly sensitive to the hyperparameter $n$. \\
         \bottomrule 
    \end{tabular}
    \vspace{4pt}
    \caption{Overview of various similarity metrics in the context of extraction attacks.}
    \label{tab:similarity_metrics}
    \vspace{-20pt}
\end{table*}
